The CARMENES search for exoplanets around M dwarfs - Photospheric parameters of target stars from high-resolution spectroscopy

The new CARMENES instrument comprises two high-resolution and high-stability spectrographs that are used to search for habitable planets around M dwarfs in the visible and near-infrared regime via the Doppler technique. Characterising our target sample is important for constraining the physical properties of any planetary systems that are detected. The aim of this paper is to determine the fundamental stellar parameters of the CARMENES M-dwarf target sample from high-resolution spectra observed with CARMENES. We also include several M-dwarf spectra observed with other high-resolution spectrographs, that is CAFE, FEROS, and HRS, for completeness. We used a {chi}^2 method to derive the stellar parameters effective temperature T_eff, surface gravity log g, and metallicity [Fe/H] of the target stars by fitting the most recent version of the PHOENIX-ACES models to high-resolution spectroscopic data. These stellar atmosphere models incorporate a new equation of state to describe spectral features of low-temperature stellar atmospheres. Since T_eff, log g, and [Fe/H] show degeneracies, the surface gravity is determined independently using stellar evolutionary models. We derive the stellar parameters for a total of 300 stars. The fits achieve very good agreement between the PHOENIX models and observed spectra. We estimate that our method provides parameters with uncertainties of {sigma} T_eff = 51 K, {sigma} log g = 0.07, and {sigma} [Fe/H] = 0.16, and show that atmosphere models for low-mass stars have significantly improved in the last years. Our work also provides an independent test of the new PHOENIX-ACES models, and a comparison for other methods using low-resolution spectra. In particular, our effective temperatures agree well with literature values, while metallicities determined with our method exhibit a larger spread when compared to literature results.

==> hires <==
@ARTICLE{Aceituno2013,
   author = {{Aceituno}, J. and {S{\'a}nchez}, S.~F. and {Grupp}, F. and 
	{Lillo}, J. and {Hern{\'a}n-Obispo}, M. and {Benitez}, D. and 
	{Montoya}, L.~M. and {Thiele}, U. and {Pedraz}, S. and {Barrado}, D. and 
	{Dreizler}, S. and {Bean}, J.},
    title = "{CAFE: Calar Alto Fiber-fed {\'E}chelle spectrograph}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1301.2066},
 primaryClass = "astro-ph.IM",
 keywords = {instrumentation: spectrographs, methods: observational, methods: data analysis, techniques: spectroscopic},
     year = 2013,
    month = apr,
   volume = 552,
      eid = {A31},
    pages = {A31},
      doi = {10.1051/0004-6361/201220361},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...552A..31A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Allard2012a,
   author = {{Allard}, F. and {Homeier}, D. and {Freytag}, B.},
    title = "{Models of very-low-mass stars, brown dwarfs and exoplanets}",
  journal = {Philosophical Transactions of the Royal Society of London Series A},
archivePrefix = "arXiv",
   eprint = {1112.3591},
 primaryClass = "astro-ph.SR",
     year = 2012,
    month = jun,
   volume = 370,
    pages = {2765-2777},
      doi = {10.1098/rsta.2011.0269},
   adsurl = {http://adsabs.harvard.edu/abs/2012RSPTA.370.2765A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Allard2012b,
   author = {{Allard}, F. and {Homeier}, D. and {Freytag}, B. and {Sharp}, C.~M.
	},
    title = "{Atmospheres From Very Low-Mass Stars to Extrasolar Planets}",
booktitle = {EAS Publications Series},
     year = 2012,
   series = {EAS Publications Series},
   volume = 57,
archivePrefix = "arXiv",
   eprint = {1206.1021},
 primaryClass = "astro-ph.SR",
   editor = {{Reyl{\'e}}, C. and {Charbonnel}, C. and {Schultheis}, M.},
    month = nov,
    pages = {3},
      doi = {10.1051/eas/1257001},
   adsurl = {http://adsabs.harvard.edu/abs/2012EAS....57....3A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Allard2011,
   author = {{Allard}, F. and {Homeier}, D. and {Freytag}, B.},
    title = "{Model Atmospheres From Very Low Mass Stars to Brown Dwarfs}",
booktitle = {16th Cambridge Workshop on Cool Stars, Stellar Systems, and the Sun},
     year = 2011,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 448,
archivePrefix = "arXiv",
   eprint = {1011.5405},
 primaryClass = "astro-ph.SR",
   editor = {{Johns-Krull}, C. and {Browning}, M.~K. and {West}, A.~A.},
    month = dec,
    pages = {91},
   adsurl = {http://adsabs.harvard.edu/abs/2011ASPC..448...91A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Allard2001,
   author = {{Allard}, F. and {Hauschildt}, P.~H. and {Alexander}, D.~R. and 
	{Tamanai}, A. and {Schweitzer}, A.},
    title = "{The Limiting Effects of Dust in Brown Dwarf Model Atmospheres}",
  journal = {\apj},
   eprint = {astro-ph/0104256},
 keywords = {Stars: Atmospheres, Stars: Fundamental Parameters, Stars: Low-Mass, Brown Dwarfs},
     year = 2001,
    month = jul,
   volume = 556,
    pages = {357-372},
      doi = {10.1086/321547},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...556..357A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Alonso2015,
   author = {{Alonso-Floriano}, F.~J. and {Morales}, J.~C. and {Caballero}, J.~A. and 
	{Montes}, D. and {Klutsch}, A. and {Mundt}, R. and {Cort{\'e}s-Contreras}, M. and 
	{Ribas}, I. and {Reiners}, A. and {Amado}, P.~J. and {Quirrenbach}, A. and 
	{Jeffers}, S.~V.},
    title = "{CARMENES input catalogue of M dwarfs. I. Low-resolution spectroscopy with CAFOS}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1502.07580},
 primaryClass = "astro-ph.SR",
 keywords = {stars: activity, stars: late-type, stars: low-mass},
     year = 2015,
    month = may,
   volume = 577,
      eid = {A128},
    pages = {A128},
      doi = {10.1051/0004-6361/201525803},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...577A.128A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Amado2013,
   author = {{Amado}, P.~J. and {Quirrenbach}, A. and {Caballero}, J.~A. and 
	{Mandel}, H. and {Ribas}, I. and {Reiners}, A. and {Sanchez-Carrasco}, M.~A. and 
	{Seifert}, W. and {Mundt}, R. and {Carmenes Consortium}},
    title = "{CARMENES: A radial-velocity survey for terrestrial planets in the habitable zones of M dwarfs. A historical overview}",
booktitle = {Highlights of Spanish Astrophysics VII},
     year = 2013,
archivePrefix = "arXiv",
   eprint = {1210.5465},
 primaryClass = "astro-ph.IM",
   editor = {{Guirado}, J.~C. and {Lara}, L.~M. and {Quilis}, V. and {Gorgas}, J.
	},
    month = may,
    pages = {842-847},
   adsurl = {http://adsabs.harvard.edu/abs/2013hsa7.conf..842A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Andersen2015,
   author = {{Andersen}, J.~M. and {Korhonen}, H.},
    title = "{Stellar activity as noise in exoplanet detection - II. Application to M dwarfs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1501.01302},
 primaryClass = "astro-ph.SR",
 keywords = {techniques: radial velocities, stars: activity, stars: low-mass, planetary systems, stars: rotation, starspots},
     year = 2015,
    month = apr,
   volume = 448,
    pages = {3053-3069},
      doi = {10.1093/mnras/stu2731},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.448.3053A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Angelov1996,
   author = {{Angelov}, T.},
    title = "{Surface gravity along the main sequence.}",
  journal = {Bulletin Astronomique de Belgrade},
 keywords = {Main-Sequence Stars: Surface Gravity},
     year = 1996,
    month = nov,
   volume = 154,
    pages = {13-16},
   adsurl = {http://adsabs.harvard.edu/abs/1996BABel.154...13A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Antonova2013,
   author = {{Antonova}, A. and {Hallinan}, G. and {Doyle}, J.~G. and {Yu}, S. and 
	{Kuznetsov}, A. and {Metodieva}, Y. and {Golden}, A. and {Cruz}, K.~L.
	},
    title = "{Volume-limited radio survey of ultracool dwarfs}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1212.3464},
 primaryClass = "astro-ph.SR",
 keywords = {stars: low-mass, brown dwarfs, radiation mechanisms: general, radio continuum: stars, masers},
     year = 2013,
    month = jan,
   volume = 549,
      eid = {A131},
    pages = {A131},
      doi = {10.1051/0004-6361/201118583},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...549A.131A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Artigau2014,
   author = {{Artigau}, {\'E}. and {Kouach}, D. and {Donati}, J.-F. and {Doyon}, R. and 
	{Delfosse}, X. and {Baratchart}, S. and {Lacombe}, M. and {Moutou}, C. and 
	{Rabou}, P. and {Par{\`e}s}, L.~P. and {Micheau}, Y. and {Thibault}, S. and 
	{Reshetov}, V.~A. and {Dubois}, B. and {Hernandez}, O. and {Vall{\'e}e}, P. and 
	{Wang}, S.-Y. and {Dolon}, F. and {Pepe}, F.~A. and {Bouchy}, F. and 
	{Striebig}, N. and {H{\'e}nault}, F. and {Loop}, D. and {Saddlemyer}, L. and 
	{Barrick}, G. and {Vermeulen}, T. and {Dupieux}, M. and {H{\'e}brard}, G. and 
	{Boisse}, I. and {Martioli}, E. and {Alencar}, S.~H.~P. and 
	{do Nascimento}, J.-D. and {Figueira}, P.},
    title = "{SPIRou: the near-infrared spectropolarimeter/high-precision velocimeter for the Canada-France-Hawaii telescope}",
booktitle = {Ground-based and Airborne Instrumentation for Astronomy V},
     year = 2014,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 9147,
archivePrefix = "arXiv",
   eprint = {1406.6992},
 primaryClass = "astro-ph.IM",
    month = jul,
      eid = {914715},
    pages = {914715},
      doi = {10.1117/12.2055663},
   adsurl = {http://adsabs.harvard.edu/abs/2014SPIE.9147E..15A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Asplund2009,
   author = {{Asplund}, M. and {Grevesse}, N. and {Sauval}, A.~J. and {Scott}, P.
	},
    title = "{The Chemical Composition of the Sun}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {0909.0948},
 primaryClass = "astro-ph.SR",
     year = 2009,
    month = sep,
   volume = 47,
    pages = {481-522},
      doi = {10.1146/annurev.astro.46.060407.145222},
   adsurl = {http://adsabs.harvard.edu/abs/2009ARA%26A..47..481A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Baraffe1998,
   author = {{Baraffe}, I. and {Chabrier}, G. and {Allard}, F. and {Hauschildt}, P.~H.
	},
    title = "{Evolutionary models for solar metallicity low-mass stars: mass-magnitude relationships and color-magnitude diagrams}",
  journal = {\aap},
   eprint = {astro-ph/9805009},
 keywords = {STARS: LOW-MASS, BROWN DWARFS, STARS: EVOLUTION, STARS: HERTZSPRUNG-RUSSEL (HR) AND C-M DIAGRAMS, STARS: INTERIORS, STARS: ATMOSPHERES},
     year = 1998,
    month = sep,
   volume = 337,
    pages = {403-412},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26A...337..403B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Baraffe2015,
   author = {{Baraffe}, I. and {Homeier}, D. and {Allard}, F. and {Chabrier}, G.
	},
    title = "{New evolutionary models for pre-main sequence and main sequence low-mass stars down to the hydrogen-burning limit}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1503.04107},
 primaryClass = "astro-ph.SR",
 keywords = {stars: evolution, stars: low-mass, stars: pre-main sequence, Hertzsprung-Russell and C-M diagrams, convection},
     year = 2015,
    month = may,
   volume = 577,
      eid = {A42},
    pages = {A42},
      doi = {10.1051/0004-6361/201425481},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...577A..42B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Benedict2016,
   author = {{Benedict}, G.~F. and {Henry}, T.~J. and {Franz}, O.~G. and 
	{McArthur}, B.~E. and {Wasserman}, L.~H. and {Jao}, W.-C. and 
	{Cargile}, P.~A. and {Dieterich}, S.~B. and {Bradley}, A.~J. and 
	{Nelan}, E.~P. and {Whipple}, A.~L.},
    title = "{The Solar Neighborhood. XXXVII: The Mass-Luminosity Relation for Main-sequence M Dwarfs}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1608.04775},
 primaryClass = "astro-ph.SR",
 keywords = {astrometry, binaries: close, stars: distances, stars: late-type, techniques: interferometric, techniques: radial velocities},
     year = 2016,
    month = nov,
   volume = 152,
      eid = {141},
    pages = {141},
      doi = {10.3847/0004-6256/152/5/141},
   adsurl = {http://adsabs.harvard.edu/abs/2016AJ....152..141B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Boyajian2012,
   author = {{Boyajian}, T.~S. and {von Braun}, K. and {van Belle}, G. and 
	{McAlister}, H.~A. and {ten Brummelaar}, T.~A. and {Kane}, S.~R. and 
	{Muirhead}, P.~S. and {Jones}, J. and {White}, R. and {Schaefer}, G. and 
	{Ciardi}, D. and {Henry}, T. and {L{\'o}pez-Morales}, M. and 
	{Ridgway}, S. and {Gies}, D. and {Jao}, W.-C. and {Rojas-Ayala}, B. and 
	{Parks}, J.~R. and {Sturmann}, L. and {Sturmann}, J. and {Turner}, N.~H. and 
	{Farrington}, C. and {Goldfinger}, P.~J. and {Berger}, D.~H.
	},
    title = "{Stellar Diameters and Temperatures. II. Main-sequence K- and M-stars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1208.2431},
 primaryClass = "astro-ph.SR",
 keywords = {Hertzsprung-Russell and C-M diagrams, infrared: stars, planetary systems, stars: atmospheres, stars: fundamental parameters, stars: general, stars: late-type, stars: low-mass, techniques: high angular resolution, techniques: interferometric},
     year = 2012,
    month = oct,
   volume = 757,
      eid = {112},
    pages = {112},
      doi = {10.1088/0004-637X/757/2/112},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...757..112B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Browning2010,
   author = {{Browning}, M.~K. and {Basri}, G. and {Marcy}, G.~W. and {West}, A.~A. and 
	{Zhang}, J.},
    title = "{Rotation and Magnetic Activity in a Sample of M-Dwarfs}",
  journal = {\aj},
 keywords = {stars: activity, stars: low-mass, brown dwarfs, stars: rotation},
     year = 2010,
    month = feb,
   volume = 139,
    pages = {504-518},
      doi = {10.1088/0004-6256/139/2/504},
   adsurl = {http://adsabs.harvard.edu/abs/2010AJ....139..504B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Burrows1997,
   author = {{Burrows}, A. and {Marley}, M. and {Hubbard}, W.~B. and {Lunine}, J.~I. and 
	{Guillot}, T. and {Saumon}, D. and {Freedman}, R. and {Sudarsky}, D. and 
	{Sharp}, C.},
    title = "{A Nongray Theory of Extrasolar Giant Planets and Brown Dwarfs}",
  journal = {\apj},
   eprint = {astro-ph/9705201},
 keywords = {Stars: Planetary Systems, Stars: Atmospheres, stars: interiors -- stars: low-mass, brown dwarfs},
     year = 1997,
    month = dec,
   volume = 491,
    pages = {856-875},
      doi = {10.1086/305002},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...491..856B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Caballero2016a,
   author = {{Caballero}, J.~A. and {Cort{\'e}s-Contreras}, M. and {Alonso-Floriano}, F.~J. and 
	{Montes}, D. and {Quirrenbach}, A. and {Amado}, P.~J. and {Ribas}, I. and 
	{Reiners}, A. and {Abellan}, F.~J. and {B{\'e}jar}, V.~J.~S. and 
	{Brinkm{\"o}ller}, M. and {Czesla}, S. and {Dorda}, R. and {Gallardo}, I. and 
	{Gonz{\'a}lez-{\'A}lvarez}, E. and {Hidalgo}, D. and {Holgado}, G. and 
	{Jeffers}, S.~V. and {Kim}, M. and {Klutsch}, A. and {Lamert}, A. and 
	{Llamas}, M. and {L{\'o}pez-Santiago}, J. and {Mart{\'{\i}}nez-Rodr{\'{\i}}guez}, H. and 
	{Morales}, J.~C. and {Mundt}, R. and {Passegger}, V.~M. and 
	{Sch{\"o}fer}, P. and {Seifert}, W. and {Zechmeister}, M.},
    title = "{Carmencita, The CARMENES Input Catalogue of Bright, Nearby M Dwarfs}",
 keywords = {stars: late-type, stars: low-mass, planetary systems, astronomical data bases, instrumentation: spectrographs},
booktitle = {19th Cambridge Workshop on Cool Stars, Stellar Systems, and the Sun (CS19)},
     year = 2016,
    month = aug,
      eid = {148},
    pages = {148},
      doi = {10.5281/zenodo.60060},
   adsurl = {http://adsabs.harvard.edu/abs/2016csss.confE.148C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Caballero2016b,
   author = {{Caballero}, J.~A. and {Gu{\`a}rdia}, J. and {L{\'o}pez del Fresno}, M. and 
	{Zechmeister}, M. and {de Juan}, E. and {Alonso-Floriano}, F.~J. and 
	{Amado}, P.~J. and {Colom{\'e}}, J. and {Cort{\'e}s-Contreras}, M. and 
	{Garc{\'{\i}}a-Piquer}, {\'A}. and {Gesa}, L. and {de Guindos}, E. and 
	{Hagen}, H.-J. and {Helmling}, J. and {Hern{\'a}ndez Casta{\~n}o}, L. and 
	{K{\"u}rster}, M. and {L{\'o}pez-Santiago}, J. and {Montes}, D. and 
	{Morales Mu{\~n}oz}, R. and {Pavlov}, A. and {Quirrenbach}, A. and 
	{Reiners}, A. and {Ribas}, I. and {Seifert}, W. and {Solano}, E.
	},
    title = "{CARMENES: data flow}",
booktitle = {Observatory Operations: Strategies, Processes, and Systems VI},
     year = 2016,
   series = {\procspie},
   volume = 9910,
    month = jul,
      eid = {99100E},
    pages = {99100E},
      doi = {10.1117/12.2233574},
   adsurl = {http://adsabs.harvard.edu/abs/2016SPIE.9910E..0EC},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ChabrierBaraffe2000,
   author = {{Chabrier}, G. and {Baraffe}, I.},
    title = "{Theory of Low-Mass Stars and Substellar Objects}",
  journal = {\araa},
   eprint = {astro-ph/0006383},
 keywords = {STARS: FUNDAMENTAL PARAMETERS, STARS: LOW MASS, BROWN DWARFS, STARS: CATACLYSMIC VARIABLES, STARS: LUMINOSITY FUNCTION, MASS FUNCTION, STARS: PLANETARY SYSTEMS, GALAXY: STELLAR CONTENT},
     year = 2000,
   volume = 38,
    pages = {337-377},
      doi = {10.1146/annurev.astro.38.1.337},
   adsurl = {http://adsabs.harvard.edu/abs/2000ARA%26A..38..337C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Claret2012,
   author = {{Claret}, A. and {Hauschildt}, P.~H. and {Witte}, S.},
    title = "{New limb-darkening coefficients for PHOENIX/1D model atmospheres. I. Calculations for 1500 K {\le} T$_{eff}$ {\le} 4800 K Kepler, CoRot, Spitzer, uvby, UBVRIJHK, Sloan, and 2MASS photometric systems}",
  journal = {\aap},
 keywords = {stars: atmospheres, binaries: eclipsing, brown dwarfs, planetary systems, stars: late-type},
     year = 2012,
    month = oct,
   volume = 546,
      eid = {A14},
    pages = {A14},
      doi = {10.1051/0004-6361/201219849},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...546A..14C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cortes2017,
   author = {{Cort{\'e}s-Contreras}, M. and {B{\'e}jar}, V.~J.~S. and {Caballero}, J.~A. and 
	{Gauza}, B. and {Montes}, D. and {Alonso-Floriano}, F.~J. and 
	{Jeffers}, S.~V. and {Morales}, J.~C. and {Reiners}, A. and 
	{Ribas}, I. and {Sch{\"o}fer}, P. and {Quirrenbach}, A. and 
	{Amado}, P.~J. and {Mundt}, R. and {Seifert}, W.},
    title = "{CARMENES input catalogue of M dwarfs. II. High-resolution imaging with FastCam}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1608.08145},
 primaryClass = "astro-ph.SR",
 keywords = {binaries : close, stars: late-type, stars: low-mass},
     year = 2017,
    month = jan,
   volume = 597,
      eid = {A47},
    pages = {A47},
      doi = {10.1051/0004-6361/201629056},
   adsurl = {http://adsabs.harvard.edu/abs/2017A%26A...597A..47C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@phdthesis{Cortes2016_2,
    title    = {CARMENES-UCM: scientific preparation, multiplicity, chromospheric activity and kinematics},
    school   = {Universidad Complutense de Madrid, Spain},
    author   = {Cort{\'e}s-Contreras, Miriam},
    year     = {2016}
}

@ARTICLE{Delfosse2000,
   author = {{Delfosse}, X. and {Forveille}, T. and {S{\'e}gransan}, D. and 
	{Beuzit}, J.-L. and {Udry}, S. and {Perrier}, C. and {Mayor}, M.
	},
    title = "{Accurate masses of very low mass stars. IV. Improved mass-luminosity relations}",
  journal = {\aap},
   eprint = {astro-ph/0010586},
 keywords = {STARS: BINARIES: GENERAL, STARS: BINARIES: SPECTROSCOPIC, STARS: BINARIES: VISUAL, STARS: LOW-MASS, BROWN DWARFS, TECHNIQUES: RADIAL VELOCITIES, STARS: LATE-TYPE},
     year = 2000,
    month = dec,
   volume = 364,
    pages = {217-224},
   adsurl = {http://adsabs.harvard.edu/abs/2000A%26A...364..217D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GaidosMann2014,
   author = {{Gaidos}, E. and {Mann}, A.~W.},
    title = "{M Dwarf Metallicities and Giant Planet Occurrence: Ironing Out Uncertainties and Systematics}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1406.4071},
 primaryClass = "astro-ph.EP",
 keywords = {planets and satellites: formation, planets and satellites: gaseous planets, stars: abundances, stars: fundamental parameters, stars: low-mass, techniques: spectroscopic},
     year = 2014,
    month = aug,
   volume = 791,
      eid = {54},
    pages = {54},
      doi = {10.1088/0004-637X/791/1/54},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...791...54G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GlebockiGnacinski2005,
   author = {{Glebocki}, R. and {Gnacinski}, P.},
    title = "{VizieR Online Data Catalog: Catalog of Stellar Rotational Velocities (Glebocki+ 2005)}",
  journal = {VizieR Online Data Catalog},
 keywords = {Rotational velocities, Associations: stellar, Clusters: open, Clusters: globular},
     year = 2005,
    month = mar,
   volume = 3244,
   adsurl = {http://adsabs.harvard.edu/abs/2005yCat.3244....0G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gustafsson2008,
   author = {{Gustafsson}, B. and {Edvardsson}, B. and {Eriksson}, K. and 
	{J{\o}rgensen}, U.~G. and {Nordlund}, {\AA}. and {Plez}, B.},
    title = "{A grid of MARCS model atmospheres for late-type stars. I. Methods and general properties}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0805.0554},
 keywords = {stars: atmospheres, Sun: abundances, stars: fundamental parameters, stars: general, stars: late-type, stars: supergiants},
     year = 2008,
    month = aug,
   volume = 486,
    pages = {951-970},
      doi = {10.1051/0004-6361:200809724},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...486..951G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hartman2015,
   author = {{Hartman}, J.~D. and {Bayliss}, D. and {Brahm}, R. and {Bakos}, G.~{\'A}. and 
	{Mancini}, L. and {Jord{\'a}n}, A. and {Penev}, K. and {Rabus}, M. and 
	{Zhou}, G. and {Butler}, R.~P. and {Espinoza}, N. and {de Val-Borro}, M. and 
	{Bhatti}, W. and {Csubry}, Z. and {Ciceri}, S. and {Henning}, T. and 
	{Schmidt}, B. and {Arriagada}, P. and {Shectman}, S. and {Crane}, J. and 
	{Thompson}, I. and {Suc}, V. and {Cs{\'a}k}, B. and {Tan}, T.~G. and 
	{Noyes}, R.~W. and {L{\'a}z{\'a}r}, J. and {Papp}, I. and {S{\'a}ri}, P.
	},
    title = "{HATS-6b: A Warm Saturn Transiting an Early M Dwarf Star, and a Set of Empirical Relations for Characterizing K and M Dwarf Planet Hosts}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1408.1758},
 primaryClass = "astro-ph.EP",
 keywords = {planetary systems, stars: individual: HATS-6, techniques: photometric, techniques: spectroscopic},
     year = 2015,
    month = may,
   volume = 149,
      eid = {166},
    pages = {166},
      doi = {10.1088/0004-6256/149/5/166},
   adsurl = {http://adsabs.harvard.edu/abs/2015AJ....149..166H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{HauschildtBaron1999,
   author = {{Hauschildt}, P.~H. and {Baron}, E.},
    title = "{Numerical solution of the expanding stellar atmosphere problem.}",
  journal = {Journal of Computational and Applied Mathematics},
   eprint = {astro-ph/9808182},
 keywords = {Stellar Atmospheres: Numerical Methods, Stellar Atmospheres: Radiative Transfer},
     year = 1999,
    month = sep,
   volume = 109,
    pages = {41-63},
   adsurl = {http://adsabs.harvard.edu/abs/1999JCoAM.109...41H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hauschildt1997,
   author = {{Hauschildt}, P.~H. and {Baron}, E. and {Allard}, F.},
    title = "{Parallel Implementation of the PHOENIX Generalized Stellar Atmosphere Program}",
  journal = {\apj},
   eprint = {astro-ph/9607087},
 keywords = {Methods: Numerical, Radiative Transfer, Stars: Atmospheres},
     year = 1997,
    month = jul,
   volume = 483,
    pages = {390-398},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...483..390H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hauschildt1999,
   author = {{Hauschildt}, P.~H. and {Allard}, F. and {Baron}, E.},
    title = "{The NextGen Model Atmosphere Grid for 3000$\lt$=T$_{eff}$$\lt$=10,000 K}",
  journal = {\apj},
   eprint = {astro-ph/9807286},
 keywords = {RADIATIVE TRANSFER, STARS: ATMOSPHERES, STARS: LATE-TYPE, Radiative Transfer, Stars: Atmospheres, Stars: Late-Type},
     year = 1999,
    month = feb,
   volume = 512,
    pages = {377-385},
      doi = {10.1086/306745},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...512..377H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hauschildt1993,
   author = {{Hauschildt}, P.~H.},
    title = "{Multi-level non-LTE radiative transfer in expanding shells.}",
  journal = {\jqsrt},
     year = 1993,
    month = sep,
   volume = 50,
    pages = {301-318},
      doi = {10.1016/0022-4073(93)90080-2},
   adsurl = {http://adsabs.harvard.edu/abs/1993JQSRT..50..301H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hauschildt1992,
   author = {{Hauschildt}, P.~H.},
    title = "{A fast operator perturbation method for the solution of the special relativistic equation of radiative transfer in spherical symmetry}",
  journal = {\jqsrt},
 keywords = {Iterative Solution, Novae, Perturbation Theory, Radiative Transfer, Relativistic Theory, Run Time (Computers), Convergence, Method Of Characteristics, Radiation Distribution, Supernovae, Wolf-Rayet Stars},
     year = 1992,
    month = jun,
   volume = 47,
    pages = {433-453},
      doi = {10.1016/0022-4073(92)90105-D},
   adsurl = {http://adsabs.harvard.edu/abs/1992JQSRT..47..433H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hebrard2014,
   author = {{H{\'e}brard}, {\'E}.~M. and {Donati}, J.-F. and {Delfosse}, X. and 
	{Morin}, J. and {Boisse}, I. and {Moutou}, C. and {H{\'e}brard}, G.
	},
    title = "{Detecting planets around active stars: impact of magnetic fields on radial velocities and line bisectors}",
  journal = {\mnras},
 keywords = {line: profiles, techniques: polarimetric, techniques: radial velocities, stars: magnetic field, starspots},
     year = 2014,
    month = sep,
   volume = 443,
    pages = {2599-2611},
      doi = {10.1093/mnras/stu1285},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.443.2599H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Houdebine2010,
   author = {{Houdebine}, E.~R.},
    title = "{Observation and modelling of main-sequence star chromospheres - XIV. Rotation of dM1 stars}",
  journal = {\mnras},
 keywords = {stars: low-mass, stars: rotation, subdwarfs},
     year = 2010,
    month = sep,
   volume = 407,
    pages = {1657-1673},
      doi = {10.1111/j.1365-2966.2010.16827.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.407.1657H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Husser2013,
   author = {{Husser}, T.-O. and {Wende-von Berg}, S. and {Dreizler}, S. and 
	{Homeier}, D. and {Reiners}, A. and {Barman}, T. and {Hauschildt}, P.~H.
	},
    title = "{A new extensive library of PHOENIX stellar atmospheres and synthetic spectra}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1303.5632},
 primaryClass = "astro-ph.SR",
 keywords = {stars: atmospheres, convection, stars: late-type},
     year = 2013,
    month = may,
   volume = 553,
      eid = {A6},
    pages = {A6},
      doi = {10.1051/0004-6361/201219058},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...553A...6H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{HusserUlbrich2014,
   author = {{Husser}, T.-O. and {Ulbrich}, K.},
    title = "{Using a model for telluric absorption in full-spectrum fits}",
 keywords = {spectral library, tellurics, full-spectrum fit },
booktitle = {Astronomical Society of India Conference Series},
     year = 2014,
   series = {Astronomical Society of India Conference Series},
   volume = 11,
archivePrefix = "arXiv",
   eprint = {1312.2450},
 primaryClass = "astro-ph.SR",
   adsurl = {http://adsabs.harvard.edu/abs/2014ASInC..11...53H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jeffers2018,
   author = {{Jeffers}, S.~V. and {Sch{\"o}fer}, P. and {Lamert}, A. and {Reiners}, A. and {Montes}, D. and {Caballero}, J. A. and 
	  {Cort{\'e}s-Contreras}, M. and {Marvin}, C.J. and {Passegger}, V.M. and {Zechmeister}, M. and {Quirrenbach}, A. and
	  {Alonso-Floriano}, F.J. and {Amado}, P.J. and {Bauer}, F.F. and {Casal}, E. and  {Diez Alonso}, E. and {Herrero}, E. and 
	  {Morales}, J.C. and {Mundt}, R. and {Ribas}, I. and {Sarmiento}, L.F.},
   title = "{CARMENES input catalogue of M dwarfs. III. Rotation and activity from high-resolution spectroscopic observations} ",
   journal = {\aap, in press, DOI10.1051/0004-6361/201629599},
   year = {2018},
   doi = {10.1051/0004-6361/201629599},
}

@ARTICLE{Jenkins2009,
   author = {{Jenkins}, J.~S. and {Ramsey}, L.~W. and {Jones}, H.~R.~A. and 
	{Pavlenko}, Y. and {Gallardo}, J. and {Barnes}, J.~R. and {Pinfield}, D.~J.
	},
    title = "{Rotational Velocities for M Dwarfs}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0908.4092},
 primaryClass = "astro-ph.SR",
 keywords = {planetary systems, stars: fundamental parameters, stars: low-mass, brown dwarfs, stars: rotation},
     year = 2009,
    month = oct,
   volume = 704,
    pages = {975-988},
      doi = {10.1088/0004-637X/704/2/975},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...704..975J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Joshi1997,
   author = {{Joshi}, M.~M. and {Haberle}, R.~M. and {Reynolds}, R.~T.},
    title = "{Simulations of the Atmospheres of Synchronously Rotating Terrestrial Planets Orbiting M Dwarfs: Conditions for Atmospheric Collapse and the Implications for Habitability}",
  journal = {\icarus},
     year = 1997,
    month = oct,
   volume = 129,
    pages = {450-465},
      doi = {10.1006/icar.1997.5793},
   adsurl = {http://adsabs.harvard.edu/abs/1997Icar..129..450J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kasting1993,
   author = {{Kasting}, J.~F. and {Whitmire}, D.~P. and {Reynolds}, R.~T.
	},
    title = "{Habitable Zones around Main Sequence Stars}",
  journal = {\icarus},
     year = 1993,
    month = jan,
   volume = 101,
    pages = {108-128},
      doi = {10.1006/icar.1993.1010},
   adsurl = {http://adsabs.harvard.edu/abs/1993Icar..101..108K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kaufer1997,
   author = {{Kaufer}, A. and {Wolf}, B. and {Andersen}, J. and {Pasquini}, L.
	},
    title = "{FEROS, the fiber-fed extended range optical spectrograph for the ESO 1.52-m telescope.}",
  journal = {The Messenger},
 keywords = {Fiber Optics: Spectrographs},
     year = 1997,
    month = sep,
   volume = 89,
    pages = {1-4},
   adsurl = {http://adsabs.harvard.edu/abs/1997Msngr..89....1K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{KenyonHartmann1995,
   author = {{Kenyon}, S.~J. and {Hartmann}, L.},
    title = "{Pre-Main-Sequence Evolution in the Taurus-Auriga Molecular Cloud}",
  journal = {\apjs},
 keywords = {INFRARED: STARS, ISM: CLOUDS, STARS: EVOLUTION, STARS: LUMINOSITY FUNCTION, MASS FUNCTION, STARS: PRE-MAIN-SEQUENCE},
     year = 1995,
    month = nov,
   volume = 101,
    pages = {117},
      doi = {10.1086/192235},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJS..101..117K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Kotani2014,
   author = {{Kotani}, T. and {Tamura}, M. and {Suto}, H. and {Nishikawa}, J. and 
	{Sato}, B. and {Aoki}, W. and {Usuda}, T. and {Kurokawa}, T. and 
	{Kashiwagi}, K. and {Nishiyama}, S. and {Ikeda}, Y. and {Hall}, D.~B. and 
	{Hodapp}, K.~W. and {Hashimoto}, J. and {Morino}, J.-I. and 
	{Okuyama}, Y. and {Tanaka}, Y. and {Suzuki}, S. and {Inoue}, S. and 
	{Kwon}, J. and {Suenaga}, T. and {Oh}, D. and {Baba}, H. and 
	{Narita}, N. and {Kokubo}, E. and {Hayano}, Y. and {Izumiura}, H. and 
	{Kambe}, E. and {Kudo}, T. and {Kusakabe}, N. and {Ikoma}, M. and 
	{Hori}, Y. and {Omiya}, M. and {Genda}, H. and {Fukui}, A. and 
	{Fujii}, Y. and {Guyon}, O. and {Harakawa}, H. and {Hayashi}, M. and 
	{Hidai}, M. and {Hirano}, T. and {Kuzuhara}, M. and {Machida}, M. and 
	{Matsuo}, T. and {Nagata}, T. and {Onuki}, H. and {Ogihara}, M. and 
	{Takami}, H. and {Takato}, N. and {Takahashi}, Y.~H. and {Tachinami}, C. and 
	{Terada}, H. and {Kawahara}, H. and {Yamamuro}, T.},
    title = "{Infrared Doppler instrument (IRD) for the Subaru telescope to search for Earth-like planets around nearby M-dwarfs}",
booktitle = {Ground-based and Airborne Instrumentation for Astronomy V},
     year = 2014,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 9147,
    month = jul,
      eid = {914714},
    pages = {914714},
      doi = {10.1117/12.2055075},
   adsurl = {http://adsabs.harvard.edu/abs/2014SPIE.9147E..14K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lammer2007,
   author = {{Lammer}, H. and {Lichtenegger}, H.~I.~M. and {Kulikov}, Y.~N. and 
	{Grie{\ss}meier}, J.-M. and {Terada}, N. and {Erkaev}, N.~V. and 
	{Biernat}, H.~K. and {Khodachenko}, M.~L. and {Ribas}, I. and 
	{Penz}, T. and {Selsis}, F.},
    title = "{Coronal Mass Ejection (CME) Activity of Low Mass M Stars as An Important Factor for The Habitability of Terrestrial Exoplanets. II. CME-Induced Ion Pick Up of Earth-like Exoplanets in Close-In Habitable Zones}",
  journal = {Astrobiology},
     year = 2007,
    month = feb,
   volume = 7,
    pages = {185-207},
      doi = {10.1089/ast.2006.0128},
   adsurl = {http://adsabs.harvard.edu/abs/2007AsBio...7..185L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Laughlin1997,
   author = {{Laughlin}, G. and {Bodenheimer}, P. and {Adams}, F.~C.},
    title = "{The End of the Main Sequence}",
  journal = {\apj},
 keywords = {Stars: Evolution, Stars: Interiors, Stars: Late-Type, Stars: Low-Mass, Brown Dwarfs},
     year = 1997,
    month = jun,
   volume = 482,
    pages = {420-432},
      doi = {10.1086/304125},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...482..420L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{LindgrenHeiter2017,
   author = {{Lindgren}, S. and {Heiter}, U.},
    title = "{Metallicity determination of M dwarfs. Expanded parameter range in metallicity and effective temperature}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1705.08785},
 primaryClass = "astro-ph.SR",
 keywords = {stars: low-mass, stars: abundances, techniques: spectroscopic},
     year = 2017,
    month = aug,
   volume = 604,
      eid = {A97},
    pages = {A97},
      doi = {10.1051/0004-6361/201730715},
   adsurl = {http://adsabs.harvard.edu/abs/2017A%26A...604A..97L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Mahadevan2014,
   author = {{Mahadevan}, S. and {Ramsey}, L.~W. and {Terrien}, R. and {Halverson}, S. and 
	{Roy}, A. and {Hearty}, F. and {Levi}, E. and {Stefansson}, G.~K. and 
	{Robertson}, P. and {Bender}, C. and {Schwab}, C. and {Nelson}, M.
	},
    title = "{The Habitable-zone Planet Finder: A status update on the development of a stabilized fiber-fed near-infrared spectrograph for the for the Hobby-Eberly telescope}",
booktitle = {Ground-based and Airborne Instrumentation for Astronomy V},
     year = 2014,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 9147,
    month = jul,
      eid = {91471G},
    pages = {91471G},
      doi = {10.1117/12.2056417},
   adsurl = {http://adsabs.harvard.edu/abs/2014SPIE.9147E..1GM},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Maldonado2015,
   author = {{Maldonado}, J. and {Affer}, L. and {Micela}, G. and {Scandariato}, G. and 
	{Damasso}, M. and {Stelzer}, B. and {Barbieri}, M. and {Bedin}, L.~R. and 
	{Biazzo}, K. and {Bignamini}, A. and {Borsa}, F. and {Claudi}, R.~U. and 
	{Covino}, E. and {Desidera}, S. and {Esposito}, M. and {Gratton}, R. and 
	{Gonz{\'a}lez Hern{\'a}ndez}, J.~I. and {Lanza}, A.~F. and {Maggio}, A. and 
	{Molinari}, E. and {Pagano}, I. and {Perger}, M. and {Pillitteri}, I. and 
	{Piotto}, G. and {Poretti}, E. and {Prisinzano}, L. and {Rebolo}, R. and 
	{Ribas}, I. and {Shkolnik}, E. and {Southworth}, J. and {Sozzetti}, A. and 
	{Su{\'a}rez Mascare{\~n}o}, A.},
    title = "{Stellar parameters of early-M dwarfs from ratios of spectral features at optical wavelengths}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1503.03010},
 primaryClass = "astro-ph.SR",
 keywords = {techniques: spectroscopic, stars: late-type, stars: low-mass, stars: fundamental parameters},
     year = 2015,
    month = may,
   volume = 577,
      eid = {A132},
    pages = {A132},
      doi = {10.1051/0004-6361/201525797},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...577A.132M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mann2013,
   author = {{Mann}, A.~W. and {Brewer}, J.~M. and {Gaidos}, E. and {L{\'e}pine}, S. and 
	{Hilton}, E.~J.},
    title = "{Prospecting in Late-type Dwarfs: A Calibration of Infrared and Visible Spectroscopic Metallicities of Late K and M Dwarfs Spanning 1.5 dex}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1211.4630},
 primaryClass = "astro-ph.SR",
 keywords = {binaries: visual, stars: abundances, stars: fundamental parameters, stars: late-type, techniques: spectroscopic},
     year = 2013,
    month = feb,
   volume = 145,
      eid = {52},
    pages = {52},
      doi = {10.1088/0004-6256/145/2/52},
   adsurl = {http://adsabs.harvard.edu/abs/2013AJ....145...52M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mann2015,
   author = {{Mann}, A.~W. and {Feiden}, G.~A. and {Gaidos}, E. and {Boyajian}, T. and 
	{von Braun}, K.},
    title = "{How to Constrain Your M Dwarf: Measuring Effective Temperature, Bolometric Luminosity, Mass, and Radius}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1501.01635},
 primaryClass = "astro-ph.SR",
 keywords = {planetary systems, stars: abundances, stars: fundamental parameters, stars: late-type, stars: low-mass, stars: statistics},
     year = 2015,
    month = may,
   volume = 804,
      eid = {64},
    pages = {64},
      doi = {10.1088/0004-637X/804/1/64},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...804...64M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MarcyChen1992,
   author = {{Marcy}, G.~W. and {Chen}, G.~H.},
    title = "{The rotation of M dwarfs}",
  journal = {\apj},
 keywords = {Dwarf Stars, K Stars, Late Stars, M Stars, Main Sequence Stars, Stellar Rotation, Absorption Spectra, Line Spectra, Radial Velocity, Stellar Spectra, Zeeman Effect},
     year = 1992,
    month = may,
   volume = 390,
    pages = {550-559},
      doi = {10.1086/171305},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...390..550M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Martinez2010,
   author = {{Mart{\'{\i}}nez-Arn{\'a}iz}, R. and {Maldonado}, J. and {Montes}, D. and 
	{Eiroa}, C. and {Montesinos}, B.},
    title = "{Chromospheric activity and rotation of FGK stars in the solar vicinity. An estimation of the radial velocity jitter}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1002.4391},
 primaryClass = "astro-ph.SR",
 keywords = {solar neighbourhood, stars: late-type, stars: activity, stars: chromospheres, stars: rotation, planetary systems},
     year = 2010,
    month = sep,
   volume = 520,
      eid = {A79},
    pages = {A79},
      doi = {10.1051/0004-6361/200913725},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...520A..79M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MohantyBasri2003,
   author = {{Mohanty}, S. and {Basri}, G.},
    title = "{Rotation and Activity in Mid-M to L Field Dwarfs}",
  journal = {\apj},
   eprint = {astro-ph/0201455},
 keywords = {Stars: Activity, Stars: Low-Mass, Brown Dwarfs, Stars: Rotation},
     year = 2003,
    month = jan,
   volume = 583,
    pages = {451-472},
      doi = {10.1086/345097},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...583..451M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Newton2017,
   author = {{Newton}, E.~R. and {Irwin}, J. and {Charbonneau}, D. and {Berlind}, P. and 
	{Calkins}, M.~L. and {Mink}, J.},
    title = "{The H{$\alpha$} Emission of Nearby M Dwarfs and its Relation to Stellar Rotation}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1611.03509},
 primaryClass = "astro-ph.SR",
 keywords = {stars: activity, stars: low-mass, stars: rotation},
     year = 2017,
    month = jan,
   volume = 834,
      eid = {85},
    pages = {85},
      doi = {10.3847/1538-4357/834/1/85},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...834...85N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Passegger2016,
   author = {{Passegger}, V.~M. and {Wende-von Berg}, S. and {Reiners}, A.
	},
    title = "{Fundamental M-dwarf parameters from high-resolution spectra using PHOENIX ACES models. I. Parameter accuracy and benchmark stars}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1601.01877},
 primaryClass = "astro-ph.SR",
 keywords = {stars: low-mass, line: formation, stars: atmospheres, brown dwarfs, line: profiles, techniques: spectroscopic},
     year = 2016,
    month = mar,
   volume = 587,
      eid = {A19},
    pages = {A19},
      doi = {10.1051/0004-6361/201322261},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...587A..19P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@phdthesis{Passegger2017,
    title    = {Characterisation of star-planet systems},
    school   = {Georg-August-Universit\"{a}t G\"{o}ttingen, Germany},
    author   = {Passegger, Vera Maria},
    year     = {2017}
}

@ARTICLE{PecautMamajek2013,
   author = {{Pecaut}, M.~J. and {Mamajek}, E.~E.},
    title = "{Intrinsic Colors, Temperatures, and Bolometric Corrections of Pre-main-sequence Stars}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1307.2657},
 primaryClass = "astro-ph.SR",
 keywords = {open clusters and associations: individual: {$\eta$} Cha cluster TW Hydra Association {$\beta$} Pic Moving Group Tucana-Horologium Association, stars: fundamental parameters, stars: pre-main sequence},
     year = 2013,
    month = sep,
   volume = 208,
      eid = {9},
    pages = {9},
      doi = {10.1088/0067-0049/208/1/9},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJS..208....9P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PiskunovValenti2002,
   author = {{Piskunov}, N.~E. and {Valenti}, J.~A.},
    title = "{New algorithms for reducing cross-dispersed echelle spectra}",
  journal = {\aap},
 keywords = {INSTRUMENTATION: SPECTROGRAPHS, METHODS: DATA ANALYSIS, TECHNIQUES: SPECTROSCOPIC},
     year = 2002,
    month = apr,
   volume = 385,
    pages = {1095-1106},
      doi = {10.1051/0004-6361:20020175},
   adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...385.1095P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{Quirrenbach2014,
   author = {{Quirrenbach}, A. and {Amado}, P.~J. and {Caballero}, J.~A. and 
	{Mundt}, R. and {Reiners}, A. and {Ribas}, I. and {Seifert}, W. and 
	{Abril}, M. and {Aceituno}, J. and {Alonso-Floriano}, F.~J. and 
	{Ammler-von Eiff}, M. and {Antona Jim{\'e}nez}, R. and {Anwand-Heerwart}, H. and 
	{Azzaro}, M. and {Bauer}, F. and {Barrado}, D. and {Becerril}, S. and 
	{B{\'e}jar}, V.~J.~S. and {Ben{\'{\i}}tez}, D. and {Berdi{\~n}as}, Z.~M. and 
	{C{\'a}rdenas}, M.~C. and {Casal}, E. and {Claret}, A. and {Colom{\'e}}, J. and 
	{Cort{\'e}s-Contreras}, M. and {Czesla}, S. and {Doellinger}, M. and 
	{Dreizler}, S. and {Feiz}, C. and {Fern{\'a}ndez}, M. and {Galad{\'{\i}}}, D. and 
	{G{\'a}lvez-Ortiz}, M.~C. and {Garc{\'{\i}}a-Piquer}, A. and 
	{Garc{\'{\i}}a-Vargas}, M.~L. and {Garrido}, R. and {Gesa}, L. and 
	{G{\'o}mez Galera}, V. and {Gonz{\'a}lez {\'A}lvarez}, E. and 
	{Gonz{\'a}lez Hern{\'a}ndez}, J.~I. and {Gr{\"o}zinger}, U. and 
	{Gu{\`a}rdia}, J. and {Guenther}, E.~W. and {de Guindos}, E. and 
	{Guti{\'e}rrez-Soto}, J. and {Hagen}, H.-J. and {Hatzes}, A.~P. and 
	{Hauschildt}, P.~H. and {Helmling}, J. and {Henning}, T. and 
	{Hermann}, D. and {Hern{\'a}ndez Casta{\~n}o}, L. and {Herrero}, E. and 
	{Hidalgo}, D. and {Holgado}, G. and {Huber}, A. and {Huber}, K.~F. and 
	{Jeffers}, S. and {Joergens}, V. and {de Juan}, E. and {Kehr}, M. and 
	{Klein}, R. and {K{\"u}rster}, M. and {Lamert}, A. and {Lalitha}, S. and 
	{Laun}, W. and {Lemke}, U. and {Lenzen}, R. and {L{\'o}pez del Fresno}, M. and 
	{L{\'o}pez Mart{\'{\i}}}, B. and {L{\'o}pez-Santiago}, J. and 
	{Mall}, U. and {Mandel}, H. and {Mart{\'{\i}}n}, E.~L. and {Mart{\'{\i}}n-Ruiz}, S. and 
	{Mart{\'{\i}}nez-Rodr{\'{\i}}guez}, H. and {Marvin}, C.~J. and 
	{Mathar}, R.~J. and {Mirabet}, E. and {Montes}, D. and {Morales Mu{\~n}oz}, R. and 
	{Moya}, A. and {Naranjo}, V. and {Ofir}, A. and {Oreiro}, R. and 
	{Pall{\'e}}, E. and {Panduro}, J. and {Passegger}, V.-M. and 
	{P{\'e}rez-Calpena}, A. and {P{\'e}rez Medialdea}, D. and {Perger}, M. and 
	{Pluto}, M. and {Ram{\'o}n}, A. and {Rebolo}, R. and {Redondo}, P. and 
	{Reffert}, S. and {Reinhardt}, S. and {Rhode}, P. and {Rix}, H.-W. and 
	{Rodler}, F. and {Rodr{\'{\i}}guez}, E. and {Rodr{\'{\i}}guez-L{\'o}pez}, C. and 
	{Rodr{\'{\i}}guez-P{\'e}rez}, E. and {Rohloff}, R.-R. and {Rosich}, A. and 
	{S{\'a}nchez-Blanco}, E. and {S{\'a}nchez Carrasco}, M.~A. and 
	{Sanz-Forcada}, J. and {Sarmiento}, L.~F. and {Sch{\"a}fer}, S. and 
	{Schiller}, J. and {Schmidt}, C. and {Schmitt}, J.~H.~M.~M. and 
	{Solano}, E. and {Stahl}, O. and {Storz}, C. and {St{\"u}rmer}, J. and 
	{Su{\'a}rez}, J.~C. and {Ulbrich}, R.~G. and {Veredas}, G. and 
	{Wagner}, K. and {Winkler}, J. and {Zapatero Osorio}, M.~R. and 
	{Zechmeister}, M. and {Abell{\'a}n de Paco}, F.~J. and {Anglada-Escud{\'e}}, G. and 
	{del Burgo}, C. and {Klutsch}, A. and {Lizon}, J.~L. and {L{\'o}pez-Morales}, M. and 
	{Morales}, J.~C. and {Perryman}, M.~A.~C. and {Tulloch}, S.~M. and 
	{Xu}, W.},
    title = "{CARMENES instrument overview}",
booktitle = {Ground-based and Airborne Instrumentation for Astronomy V},
     year = 2014,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 9147,
    month = jul,
      eid = {91471F},
    pages = {91471F},
      doi = {10.1117/12.2056453},
   adsurl = {http://adsabs.harvard.edu/abs/2014SPIE.9147E..1FQ},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Quirrenbach2016,
   author = {{Quirrenbach}, A. and {Amado}, P.~J. and {Caballero}, J.~A. and 
	{Mundt}, R. and {Reiners}, A. and {Ribas}, I. and {Seifert}, W. and 
	{Abril}, M. and {Aceituno}, J. and {Alonso-Floriano}, F.~J. and 
	{Anwand-Heerwart}, H. and {Azzaro}, M. and {Bauer}, F. and {Barrado}, D. and 
	{Becerril}, S. and {Bejar}, V.~J.~S. and {Benitez}, D. and {Berdinas}, Z.~M. and 
	{Brinkm{\"o}ller}, M. and {Cardenas}, M.~C. and {Casal}, E. and 
	{Claret}, A. and {Colom{\'e}}, J. and {Cortes-Contreras}, M. and 
	{Czesla}, S. and {Doellinger}, M. and {Dreizler}, S. and {Feiz}, C. and 
	{Fernandez}, M. and {Ferro}, I.~M. and {Fuhrmeister}, B. and 
	{Galadi}, D. and {Gallardo}, I. and {G{\'a}lvez-Ortiz}, M.~C. and 
	{Garcia-Piquer}, A. and {Garrido}, R. and {Gesa}, L. and {G{\'o}mez Galera}, V. and 
	{Gonz{\'a}lez Hern{\'a}ndez}, J.~I. and {Gonzalez Peinado}, R. and 
	{Gr{\"o}zinger}, U. and {Gu{\`a}rdia}, J. and {Guenther}, E.~W. and 
	{de Guindos}, E. and {Hagen}, H.-J. and {Hatzes}, A.~P. and 
	{Hauschildt}, P.~H. and {Helmling}, J. and {Henning}, T. and 
	{Hermann}, D. and {Hern{\'a}ndez Arabi}, R. and {Hern{\'a}ndez Casta{\~n}o}, L. and 
	{Hern{\'a}ndez Hernando}, F. and {Herrero}, E. and {Huber}, A. and 
	{Huber}, K.~F. and {Huke}, P. and {Jeffers}, S.~V. and {de Juan}, E. and 
	{Kaminski}, A. and {Kehr}, M. and {Kim}, M. and {Klein}, R. and 
	{Kl{\"u}ter}, J. and {K{\"u}rster}, M. and {Lafarga}, M. and 
	{Lara}, L.~M. and {Lamert}, A. and {Laun}, W. and {Launhardt}, R. and 
	{Lemke}, U. and {Lenzen}, R. and {Llamas}, M. and {Lopez del Fresno}, M. and 
	{L{\'o}pez-Puertas}, M. and {L{\'o}pez-Santiago}, J. and {Lopez Salas}, J.~F. and 
	{Magan Madinabeitia}, H. and {Mall}, U. and {Mandel}, H. and 
	{Mancini}, L. and {Marin Molina}, J.~A. and {Maroto Fern{\'a}ndez}, D. and 
	{Mart{\'{\i}}n}, E.~L. and {Mart{\'{\i}}n-Ruiz}, S. and {Marvin}, C. and 
	{Mathar}, R.~J. and {Mirabet}, E. and {Montes}, D. and {Morales}, J.~C. and 
	{Morales Mu{\~n}oz}, R. and {Nagel}, E. and {Naranjo}, V. and 
	{Nowak}, G. and {Palle}, E. and {Panduro}, J. and {Passegger}, V.~M. and 
	{Pavlov}, A. and {Pedraz}, S. and {Perez}, E. and {P{\'e}rez-Medialdea}, D. and 
	{Perger}, M. and {Pluto}, M. and {Ram{\'o}n}, A. and {Rebolo}, R. and 
	{Redondo}, P. and {Reffert}, S. and {Reinhart}, S. and {Rhode}, P. and 
	{Rix}, H.-W. and {Rodler}, F. and {Rodr{\'{\i}}guez}, E. and 
	{Rodr{\'{\i}}guez L{\'o}pez}, C. and {Rohloff}, R.~R. and {Rosich}, A. and 
	{Sanchez Carrasco}, M.~A. and {Sanz-Forcada}, J. and {Sarkis}, P. and 
	{Sarmiento}, L.~F. and {Sch{\"a}fer}, S. and {Schiller}, J. and 
	{Schmidt}, C. and {Schmitt}, J.~H.~M.~M. and {Sch{\"o}fer}, P. and 
	{Schweitzer}, A. and {Shulyak}, D. and {Solano}, E. and {Stahl}, O. and 
	{Storz}, C. and {Tabernero}, H.~M. and {Tala}, M. and {Tal-Or}, L. and 
	{Ulbrich}, R.-G. and {Veredas}, G. and {Vico Linares}, J.~I. and 
	{Vilardell}, F. and {Wagner}, K. and {Winkler}, J. and {Zapatero Osorio}, M.-R. and 
	{Zechmeister}, M. and {Ammler-von Eiff}, M. and {Anglada-Escud{\'e}}, G. and 
	{del Burgo}, C. and {Garcia-Vargas}, M.~L. and {Klutsch}, A. and 
	{Lizon}, J.-L. and {Lopez-Morales}, M. and {Ofir}, A. and {P{\'e}rez-Calpena}, A. and 
	{Perryman}, M.~A.~C. and {S{\'a}nchez-Blanco}, E. and {Strachan}, J.~B.~P. and 
	{St{\"u}rmer}, J. and {Su{\'a}rez}, J.~C. and {Trifonov}, T. and 
	{Tulloch}, S.~M. and {Xu}, W.},
    title = "{CARMENES: an overview six months after first light}",
booktitle = {Ground-based and Airborne Instrumentation for Astronomy VI},
     year = 2016,
   series = {\procspie},
   volume = 9908,
    month = aug,
      eid = {990812},
    pages = {990812},
      doi = {10.1117/12.2231880},
   adsurl = {http://adsabs.harvard.edu/abs/2016SPIE.9908E..12Q},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Rajpurohit2012,
   author = {{Rajpurohit}, A.~S. and {Reyl{\'e}}, C. and {Schultheis}, M. and 
	{Allard}, F. and {Scholz}, R. and {Homeier}, D.},
    title = "{Stellar parameters of M dwarfs from low and high-resolution spectra together with new model atmospheres}",
 keywords = {stars: atmospheres, stars: fundamental parameters, stars: low-mass-brown dwarfs},
booktitle = {SF2A-2012: Proceedings of the Annual meeting of the French Society of Astronomy and Astrophysics},
     year = 2012,
   editor = {{Boissier}, S. and {de Laverny}, P. and {Nardetto}, N. and {Samadi}, R. and 
	{Valls-Gabaud}, D. and {Wozniak}, H.},
    month = dec,
    pages = {383-388},
   adsurl = {http://adsabs.harvard.edu/abs/2012sf2a.conf..383R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rajpurohit2013,
   author = {{Rajpurohit}, A.~S. and {Reyl{\'e}}, C. and {Allard}, F. and 
	{Homeier}, D. and {Schultheis}, M. and {Bessell}, M.~S. and 
	{Robin}, A.~C.},
    title = "{The effective temperature scale of M dwarfs}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1304.4072},
 primaryClass = "astro-ph.SR",
 keywords = {stars: atmospheres, stars: low-mass, stars: fundamental parameters},
     year = 2013,
    month = aug,
   volume = 556,
      eid = {A15},
    pages = {A15},
      doi = {10.1051/0004-6361/201321346},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...556A..15R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reiners2010,
   author = {{Reiners}, A. and {Bean}, J.~L. and {Huber}, K.~F. and {Dreizler}, S. and 
	{Seifahrt}, A. and {Czesla}, S.},
    title = "{Detecting Planets Around Very Low Mass Stars with the Radial Velocity Method}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0909.0002},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, stars: activity, stars: low-mass, starspots, techniques: radial velocities},
     year = 2010,
    month = feb,
   volume = 710,
    pages = {432-443},
      doi = {10.1088/0004-637X/710/1/432},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...710..432R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reiners2012,
   author = {{Reiners}, A. and {Joshi}, N. and {Goldman}, B.},
    title = "{A Catalog of Rotation and Activity in Early-M Stars}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1201.5774},
 primaryClass = "astro-ph.SR",
 keywords = {stars: activity, stars: low-mass, stars: rotation},
     year = 2012,
    month = apr,
   volume = 143,
      eid = {93},
    pages = {93},
      doi = {10.1088/0004-6256/143/4/93},
   adsurl = {http://adsabs.harvard.edu/abs/2012AJ....143...93R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Reiners2013,
   author = {{Reiners}, A. and {Shulyak}, D. and {Anglada-Escud{\'e}}, G. and 
	{Jeffers}, S.~V. and {Morin}, J. and {Zechmeister}, M. and {Kochukhov}, O. and 
	{Piskunov}, N.},
    title = "{Radial velocity signatures of Zeeman broadening}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1301.2951},
 primaryClass = "astro-ph.SR",
 keywords = {line: profiles, techniques: radial velocities, stars: activity, starspots, stars: magnetic field},
     year = 2013,
    month = apr,
   volume = 552,
      eid = {A103},
    pages = {A103},
      doi = {10.1051/0004-6361/201220437},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...552A.103R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reiners2017,
   author = {{Reiners}, A. and {Zechmeister}, M. and {Caballero}, J.~A. and 
	{Ribas}, I. and {Morales}, J.~C. and {Jeffers}, S.~V. and {Sch{\"o}fer}, P. and 
	{Tal-Or}, L. and {Quirrenbach}, A. and {Amado}, P.~J. and {Kaminski}, A. and 
	{Seifert}, W. and {Abril}, M. and {Aceituno}, J. and {Alonso-Floriano}, F.~J. and 
	{Ammler-von Eiff}, M. and {Antona}, R. and {Anglada-Escud{\'e}}, G. and 
	{Anwand-Heerwart}, H. and {Arroyo-Torres}, B. and {Azzaro}, M. and 
	{Baroch}, D. and {Barrado}, D. and {Bauer}, F.~F. and {Becerril}, S. and 
	{B{\'e}jar}, V.~J.~S. and {Ben{\'{\i}}tez}, D. and {Berdi{\~n}as}, Z.~M. and 
	{Bergond}, G. and {Bl{\"u}mcke}, M. and {Brinkm{\"o}ller}, M. and 
	{del Burgo}, C. and {Cano}, J. and {C{\'a}rdenas V{\'a}zquez}, M.~C. and 
	{Casal}, E. and {Cifuentes}, C. and {Claret}, A. and {Colom{\'e}}, J. and 
	{Cort{\'e}s-Contreras}, M. and {Czesla}, S. and {D{\'{\i}}ez-Alonso}, E. and 
	{Dreizler}, S. and {Feiz}, C. and {Fern{\'a}ndez}, M. and {Ferro}, I.~M. and 
	{Fuhrmeister}, B. and {Galad{\'{\i}}-Enr{\'{\i}}quez}, D. and 
	{Garcia-Piquer}, A. and {Garc{\'{\i}}a Vargas}, M.~L. and {Gesa}, L. and 
	{G{\'o}mez}, V. and {Galera} and {Gonz{\'a}lez Hern{\'a}ndez}, J.~I. and 
	{Gonz{\'a}lez-Peinado}, R. and {Gr{\"o}zinger}, U. and {Grohnert}, S. and 
	{Gu{\`a}rdia}, J. and {Guenther}, E.~W. and {Guijarro}, A. and 
	{de Guindos}, E. and {Guti{\'e}rrez-Soto}, J. and {Hagen}, H.-J. and 
	{Hatzes}, A.~P. and {Hauschildt}, P.~H. and {Hedrosa}, R.~P. and 
	{Helmling}, J. and {Henning}, T. and {Hermelo}, I. and {Hern{\'a}ndez Arab{\'{\i}}}, R. and 
	{Hern{\'a}ndez Casta{\~n}o}, L. and {Hern{\'a}ndez Hernando}, F. and 
	{Herrero}, E. and {Huber}, A. and {Huke}, P. and {Johnson}, E. and 
	{de Juan}, E. and {Kim}, M. and {Klein}, R. and {Kl{\"u}ter}, J. and 
	{Klutsch}, A. and {K{\"u}rster}, M. and {Lafarga}, M. and {Lamert}, A. and 
	{Lamp{\'o}n}, M. and {Lara}, L.~M. and {Laun}, W. and {Lemke}, U. and 
	{Lenzen}, R. and {Launhardt}, R. and {L{\'o}pez del Fresno}, M. and 
	{L{\'o}pez-Gonz{\'a}lez}, J. and {L{\'o}pez-Puertas}, M. and 
	{L{\'o}pez Salas}, J.~F. and {L{\'o}pez-Santiago}, J. and {Luque}, R. and 
	{Mag{\'a}n Madinabeitia}, H. and {Mall}, U. and {Mancini}, L. and 
	{Mandel}, H. and {Marfil}, E. and {Mar{\'{\i}}n Molina}, J.~A. and 
	{Maroto}, D. and {Fern{\'a}ndez} and {Mart{\'{\i}}n}, E.~L. and 
	{Mart{\'{\i}}n-Ruiz}, S. and {Marvin}, C.~J. and {Mathar}, R.~J. and 
	{Mirabet}, E. and {Montes}, D. and {Moreno-Raya}, M.~E. and 
	{Moya}, A. and {Mundt}, R. and {Nagel}, E. and {Naranjo}, V. and 
	{Nortmann}, L. and {Nowak}, G. and {Ofir}, A. and {Oreiro}, R. and 
	{Pall{\'e}}, E. and {Panduro}, J. and {Pascual}, J. and {Passegger}, V.~M. and 
	{Pavlov}, A. and {Pedraz}, S. and {P{\'e}rez-Calpena}, A. and 
	{P{\'e}rez Medialdea}, D. and {Perger}, M. and {Perryman}, M.~A.~C. and 
	{Pluto}, M. and {Rabaza}, O. and {Ram{\'o}n}, A. and {Rebolo}, R. and 
	{Redondo}, P. and {Reffert}, S. and {Reinhart}, S. and {Rhode}, P. and 
	{Rix}, H.-W. and {Rodler}, F. and {Rodr{\'{\i}}guez}, E. and 
	{Rodr{\'{\i}}guez-L{\'o}pez}, C. and {Rodr{\'{\i}}guez Trinidad}, A. and 
	{Rohloff}, R.-R. and {Rosich}, A. and {Sadegi}, S. and {S{\'a}nchez-Blanco}, E. and 
	{S{\'a}nchez Carrasco}, M.~A. and {S{\'a}nchez-L{\'o}pez}, A. and 
	{Sanz-Forcada}, J. and {Sarkis}, P. and {Sarmiento}, L.~F. and 
	{Sch{\"a}fer}, S. and {Schmitt}, J.~H.~M.~M. and {Schiller}, J. and 
	{Schweitzer}, A. and {Solano}, E. and {Stahl}, O. and {Strachan}, J.~B.~P. and 
	{St{\"u}rmer}, J. and {Su{\'a}rez}, J.~C. and {Tabernero}, H.~M. and 
	{Tala}, M. and {Trifonov}, T. and {Tulloch}, S.~M. and {Ulbrich}, R.~G. and 
	{Veredas}, G. and {Vico Linares}, J.~I. and {Vilardell}, F. and 
	{Wagner}, K. and {Winkler}, J. and {Wolthoff}, V. and {Xu}, W. and 
	{Yan}, F. and {Zapatero Osorio}, M.~R.},
    title = "{The CARMENES search for exoplanets around M dwarfs: High-resolution optical and near-infrared spectroscopy of 324 survey stars}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1711.06576},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
     year = 2017,
    month = nov,
    doi = {10.1051/0004-6361/201732054},
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv171106576R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ReinersBasri2007,
   author = {{Reiners}, A. and {Basri}, G.},
    title = "{The First Direct Measurements of Surface Magnetic Fields on Very Low Mass Stars}",
  journal = {\apj},
   eprint = {astro-ph/0610365},
 keywords = {Stars: Low-Mass, Brown Dwarfs, Stars: Magnetic Fields},
     year = 2007,
    month = feb,
   volume = 656,
    pages = {1121-1135},
      doi = {10.1086/510304},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...656.1121R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{RojasAyala2012,
   author = {{Rojas-Ayala}, B. and {Covey}, K.~R. and {Muirhead}, P.~S. and 
	{Lloyd}, J.~P.},
    title = "{Metallicity and Temperature Indicators in M Dwarf K-band Spectra: Testing New and Updated Calibrations with Observations of 133 Solar Neighborhood M Dwarfs}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1112.4567},
 primaryClass = "astro-ph.SR",
 keywords = {stars: abundances, stars: fundamental parameters, stars: late-type},
     year = 2012,
    month = apr,
   volume = 748,
      eid = {93},
    pages = {93},
      doi = {10.1088/0004-637X/748/2/93},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...748...93R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@thesis{Schoefer2015,
  author = {{Sch{\"o}fer}, P.},
  title = "{MSc Thesis, Georg-August Universit{\"a}t G{\"o}ttingen, Germany}",
  school = {Georg-August Universit{\"a}t G{\"o}ttingen, Germany},
  year = 2015,
  month = oct,
}

@ARTICLE{Souto2017,
   author = {{Souto}, D. and {Cunha}, K. and {Garc{\'{\i}}a-Hern{\'a}ndez}, D.~A. and 
	{Zamora}, O. and {Allende Prieto}, C. and {Smith}, V.~V. and 
	{Mahadevan}, S. and {Blake}, C. and {Johnson}, J.~A. and {J{\"o}nsson}, H. and 
	{Pinsonneault}, M. and {Holtzman}, J. and {Majewski}, S.~R. and 
	{Shetrone}, M. and {Teske}, J. and {Nidever}, D. and {Schiavon}, R. and 
	{Sobeck}, J. and {Garc{\'{\i}}a P{\'e}rez}, A.~E. and {G{\'o}mez Maqueo Chew}, Y. and 
	{Stassun}, K.},
    title = "{Chemical Abundances of M-dwarfs from the APOGEE Survey. I. The Exoplanet Hosting Stars Kepler-138 and Kepler-186}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1612.01598},
 primaryClass = "astro-ph.SR",
 keywords = {infrared: stars, planetary systems, planet{\ndash}star interactions, stars: abundances, stars: fundamental parameters, stars: low-mass},
     year = 2017,
    month = feb,
   volume = 835,
      eid = {239},
    pages = {239},
      doi = {10.3847/1538-4357/835/2/239},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...835..239S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Stahl1999,
   author = {{Stahl}, O. and {Kaufer}, A. and {Tubbesing}, S.},
    title = "{The FEROS spectrograph}",
booktitle = {Optical and Infrared Spectroscopy of Circumstellar Matter},
     year = 1999,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 188,
   editor = {{Guenther}, E. and {Stecklum}, B. and {Klose}, S.},
    pages = {331},
   adsurl = {http://adsabs.harvard.edu/abs/1999ASPC..188..331S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{StaufferHartmann1986,
   author = {{Stauffer}, J.~B. and {Hartmann}, L.~W.},
    title = "{The rotational velocities of low-mass stars}",
  journal = {\pasp},
 keywords = {Angular Velocity, Stellar Evolution, Stellar Mass, Stellar Rotation, Angular Momentum, Dwarf Stars, G Stars, Late Stars, Main Sequence Stars},
     year = 1986,
    month = dec,
   volume = 98,
    pages = {1233-1251},
      doi = {10.1086/131926},
   adsurl = {http://adsabs.harvard.edu/abs/1986PASP...98.1233S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Tull1998,
   author = {{Tull}, R.~G. and {MacQueen}, P.~J. and {Good}, J. and {Epps}, H.~W. and 
	{HET HRS Team}},
    title = "{High Resolution Spectrograph for the Hobby-Eberly Telescope}",
booktitle = {American Astronomical Society Meeting Abstracts},
     year = 1998,
   series = {Bulletin of the American Astronomical Society},
   volume = 30,
    month = dec,
      eid = {10.08},
    pages = {1263},
   adsurl = {http://adsabs.harvard.edu/abs/1998AAS...193.1008T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ValentiPiskunov1996,
   author = {{Valenti}, J.~A. and {Piskunov}, N.},
    title = "{Spectroscopy made easy: A new tool for fitting observations with synthetic spectra.}",
  journal = {\aaps},
 keywords = {RADIATIVE TRANSFER, METHODS: NUMERICAL, TECHNIQUES: SPECTROSCOPIC, STARS: FUNDAMENTAL PARAMETERS, SUN: FUNDAMENTAL PARAMETERS, ATOMIC DATA},
     year = 1996,
    month = sep,
   volume = 118,
    pages = {595-603},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26AS..118..595V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Veyette2016,
   author = {{Veyette}, M.~J. and {Muirhead}, P.~S. and {Mann}, A.~W. and 
	{Allard}, F.},
    title = "{The Physical Mechanism Behind M Dwarf Metallicity Indicators and the Role of C and O Abundances}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1605.04904},
 primaryClass = "astro-ph.SR",
 keywords = {brown dwarfs, stars: abundances, stars: atmospheres, stars: fundamental parameters, stars: late-type, stars: low-mass},
     year = 2016,
    month = sep,
   volume = 828,
      eid = {95},
    pages = {95},
      doi = {10.3847/0004-637X/828/2/95},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...828...95V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Veyette2017,
   author = {{Veyette}, M.~J. and {Muirhead}, P.~S. and {Mann}, A.~W. and 
	{Brewer}, J.~M. and {Allard}, F. and {Homeier}, D.},
    title = "{A Physically Motivated and Empirically Calibrated Method to Measure the Effective Temperature, Metallicity, and Ti Abundance of M Dwarfs}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1710.10259},
 primaryClass = "astro-ph.SR",
 keywords = {stars: abundances, stars: atmospheres, stars: fundamental parameters, stars: late-type, stars: low-mass},
     year = 2017,
    month = dec,
   volume = 851,
      eid = {26},
    pages = {26},
      doi = {10.3847/1538-4357/aa96aa},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...851...26V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vonBraun2014,
   author = {{von Braun}, K. and {Boyajian}, T.~S. and {van Belle}, G.~T. and 
	{Kane}, S.~R. and {Jones}, J. and {Farrington}, C. and {Schaefer}, G. and 
	{Vargas}, N. and {Scott}, N. and {ten Brummelaar}, T.~A. and 
	{Kephart}, M. and {Gies}, D.~R. and {Ciardi}, D.~R. and {L{\'o}pez-Morales}, M. and 
	{Mazingue}, C. and {McAlister}, H.~A. and {Ridgway}, S. and 
	{Goldfinger}, P.~J. and {Turner}, N.~H. and {Sturmann}, L.},
    title = "{Stellar diameters and temperatures - V. 11 newly characterized exoplanet host stars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1312.1792},
 primaryClass = "astro-ph.EP",
 keywords = {techniques: interferometric, stars: fundamental parameters, stars: general, stars: late-type, planetary systems, infrared: stars},
     year = 2014,
    month = mar,
   volume = 438,
    pages = {2413-2425},
      doi = {10.1093/mnras/stt2360},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.438.2413V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zechmeister2014,
   author = {{Zechmeister}, M. and {Anglada-Escud{\'e}}, G. and {Reiners}, A.
	},
    title = "{Flat-relative optimal extraction. A quick and efficient algorithm for stabilised spectrographs}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1311.5263},
 primaryClass = "astro-ph.IM",
 keywords = {instrumentation: spectrographs, methods: data analysis, techniques: image processing, techniques: radial velocities},
     year = 2014,
    month = jan,
   volume = 561,
      eid = {A59},
    pages = {A59},
      doi = {10.1051/0004-6361/201322746},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...561A..59Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zechmeister2017,
   author = {{Zechmeister}, M. and {Reiners}, A. and {Amado}, P.~J. and {Azzaro}, M. and 
	{Bauer}, F.~F. and {B{\'e}jar}, V.~J.~S. and {Caballero}, J.~A. and 
	{Guenther}, E.~W. and {Hagen}, H.-J. and {Jeffers}, S.~V. and 
	{Kaminski}, A. and {K{\"u}rster}, M. and {Launhardt}, R. and 
	{Montes}, D. and {Morales}, J.~C. and {Quirrenbach}, A. and 
	{Reffert}, S. and {Ribas}, I. and {Seifert}, W. and {Tal-Or}, L. and 
	{Wolthoff}, V.},
    title = "{Spectrum radial velocity analyser (SERVAL). High-precision radial velocities and two alternative spectral indicators}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1710.10114},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, techniques: radial velocities, techniques: spectroscopic, planets and satellites: detection},
     year = 2017,
    month = dec,
   volume = 609,
      eid = {A12},
    pages = {A12},
      doi = {10.1051/0004-6361/201731483},
   adsurl = {http://adsabs.harvard.edu/abs/2017A%26A...609A..12Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
